A Dual Process VLA: Efficient Robotic Manipulation Leveraging VLM

Vision-Language-Action (VLA) models are receiving increasing attention for their ability to enable robots to perform complex tasks by integrating visual context with linguistic commands. However, achieving efficient real-time performance remains challenging due to the high computational demands of existing models. To overcome this, we propose Dual Process VLA (DP-VLA), a hierarchical framework inspired by dual-process theory. DP-VLA utilizes a Large System 2 Model (L-Sys2) for complex reasoning and decision-making, while a Small System 1 Model (S-Sys1) handles real-time motor control and sensory processing. By leveraging Vision-Language Models (VLMs), the L-Sys2 operates at low frequencies, reducing computational overhead, while the S-Sys1 ensures fast and accurate task execution. Experimental results on the RoboCasa dataset demonstrate that DP-VLA achieves faster inference and higher task success rates, providing a scalable solution for advanced robotic applications.

==> tex/intro_jjh.tex <==
	
    %Submission to CoRL 2024 will be entirely electronic, via a web site (not email). Information about the submission process and \LaTeX{} templates are available on the conference web site at \url{https://corl2024.org/}. For camera ready submission, use the \texttt{final} option for the \texttt{\textbackslash usepackage} command. 


    % Related Works: RT Series (3Hz), OpenVLA (LLaMA 7B), Octo (Diffusion-based) --> 모두 느림 

    % 문제점: 매우 느린 속도, LLM에 드는 거대 장비


    % Motivation: Human Brain? --> System 1 & 2

    % OpenVLA 시작: A key weakness of learned policies for robotic manipulation is their inability to generalize beyond their training data: while existing policies trained for individual skills or language instructions have the capacity to extrapolate behaviors to new initial conditions such as object positions or lighting [2, 3], they lack robustness to scene distractors or novel objects [4, 5] and struggle to execute unseen task instructions [6, 7]. Yet beyond robotics, existing foundation models for vision and language such as CLIP [8], SigLIP [9], and Llama 2 [10] are capable of these types of generalization and more, stemming from the priors captured by their Internet-scale pretraining datasets. While reproducing this scale of pretraining for robotics is still an open challenge — even the largest robot manipulation datasets [1, 11] only have 100K to 1M examples – this imbalance suggests an opportunity: using existing foundation models for vision and language as a core building block for training robotic policies that can generalize to objects, scenes, and tasks beyond their training data.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Recently, there have been remarkable advancements in the research of policy learning for robotic manipulation.

% Given a task instruction from a user, policy models generate intermediate robot actions via the following steps: 1) understanding the given instruction, 2) analyzing the current visual data in terms of the given task, and 3) predicting the required actions to perform the task. Many studies have called these models vision-language-action models (VLAs). However, VLA is highly challenging because it requires a combination of multiple intelligences (i.e., speech-to-text, text understanding, vision understanding, and action generation). Without harmonization of these high-level techniques, robots cannot succeed in the given mission. Despite the challenge, recent VLA studies have reported promising results, indicating applicability in real-world scenarios.

% One reason for the improvement is the availability of huge amounts of datasets and realistic simulations. With the development of tele-operation and graphics techniques, it has become possible to collect robot action datasets easily. Through tele-operation, humans can control a robot, and the action trajectories can be easily recorded. Many portions of the Open-X-Embodiment and DROID datasets were collected through this process. Furthermore, rendering techniques help to collect human data even without a real robot, enrich the recorded data with varying environments and viewpoints, and facilitate easy validation of VLA models.

% The second key advancement in VLA is generality. Recent VLA studies have empirically demonstrated general applicability even to unseen instructions. Importantly, this generality has been built upon large language models (LLMs) and vision-language models (VLMs), which provide general understanding capabilities for the given instructions. RT-2 and RT-X \cite{???} initially proposed the concept of VLM-based robot action generation. Subsequently, several studies, such as OpenVLA \cite{???} and LLARVA \cite{???}, have proven the feasibility.

% Third, data synthesizing techniques have also contributed. Many recent studies, such as Diffusion Policy \cite{??} and Octo \cite{??}, have adopted diffusion models as their prediction methods instead of regression or classification. Diffusion models are widely known for generating realistic and diverse data, and VLA studies leverage this property to predict realistic and diverse robot actions.

% However, a critical drawback of recent VLA methods is the processing time. LLMs require heavy computational cost, and the cost increases with the length of the instruction. When prior works are applied to practical robots, their motions appear highly unnatural and choppy due to this limitation.

% In this paper, we employ the concepts of System 1 and System 2 to divide VLA into two separate parts: 1) an in-depth understanding module, and 2) a lightweight module to predict intermediate actions with shallow understanding. The first module provides understanding of long-term components (i.e., instruction and initial observation of the environment), and the second module processes short-term components (i.e., current motion and visual observation). Therefore, by scheduling the modules—processing the first module less frequently and the second module more frequently—we can reduce redundant computations and make the robot's motion more natural.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    % Recently, there have been remarkable advancement in the research of policy learning for robotic manipulation. 

    
    % Given a task instruction from an user, policy model generates intermediate robot actions via following steps: 1) understanding the given instruction, 2) analyzing the current visual data in terms of the given task, and 3) prediction of required actions to do the task. Many studies have called these models as vision-language-action models (VLAs). However, this VLA is highly challenging because it requires a composite of multiple intelligence (i.e., speech-to-text, text understanding, vision understanding, and action generation). Without harmonization of the high-level techniques, robots cannot succeed in the given mission. Despite the challenge, recent VLA studies have reported some promising results to be applicable in reality.   

    % One reason of the improvement is huge amount of dataset and realistic simulation. With development of tele-operation and graphics techniques, it becomes possible to collect robot action dataset easily. By tele-operation, human can control a robot and the action trajectories can be easily recorded. Many portion of Open-X-Embodiment and DROID datasets were collected as this process. Further, rendering technique help to collect the human data even without the real robot, enrich the recorded data with varying environments and viewpoints, validate VLA models easily. 
    


    % The second key advancement of VLA is the generality. Recent VLA studies empirically demonstrate the general applicability even to unseen instructions. Importantly, the generality has been built upon large language models (LLMs) and vision-language models (VLMs), which give the general understanding ability about the given instruction. RT-2 and RT-X \cite{???} initially proposed the concept of VLM-based robot action generation. Then, several studies, such as OpenVLA \cite{???} or LLARVA \cite{???}, have proved the feasibility.  
     
    % Third, the data synthesizing technique also have some contribution. Many recent studies, such as diffusion policy \cite{??} and octo \cite{??}, have adopted diffusion models as their prediction method instead of regression or classification. Diffusion models are widely known as a method that can generate realistic and diverse data, and the VLA studies inherit the property to predict realistic and diverse robot actions. 
    
    % However, a critical drawback of the recent VLA is the processing time. LLMs requires heavy computation cost, and the cost becomes larger by the length of the instruction. When prior works are applied into practical robot, their motions look highly unnatural and and choppy due to this limitation.
    
    % In this paper, we employed the concept of System 1 and System 2 to divide VLA into two separate parts: 1) in-depth understanding module, and 2) light module to predict the intermediate action with shallow understanding. The first module gives the understanding about long-term components (i.e., instruction and initial observation about the environment), and the second one process the short-term components (i.e., current motion and visual observation). Therefore, it is possible to reduce the redundant computations and make the robot motion more natural via scheduling the modules (low-frequent process for the first module and frequent process for the second one).  

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In recent years, significant advancements have been made in policy learning for robotic manipulation. Policy models, when provided with a user's task instruction, generate intermediate robot actions through the following steps: (1) comprehending the instruction, (2) analyzing current visual data in the context of the task, and (3) predicting the necessary actions to execute the task. These models are often referred to in the literature as vision-language-action (VLA) models.

Developing effective VLA models is highly challenging due to the requirement of integrating multiple intelligent processes—including speech-to-text conversion, natural language understanding, visual perception, and action generation. Without seamless integration of these advanced techniques, robots cannot successfully accomplish the assigned missions. Nevertheless, recent studies in VLA have demonstrated promising results, suggesting potential applicability in real-world scenarios.

One contributing factor to these improvements is the availability of large-scale datasets and realistic simulations. Advances in tele-operation and graphics technologies have made it easier to collect robot action datasets. Through tele-operation, humans can control robots, and the resulting action trajectories can be readily recorded. Significant portions of datasets like Open-X-Embodiment and DROID have been collected using this approach. Moreover, rendering techniques enable the collection of human data without the need for a physical robot, enriching the recorded data with diverse environments and viewpoints, and facilitating efficient validation of VLA models.

A second key advancement in VLA is the enhancement of generality. Recent studies have empirically demonstrated that VLA models can generalize to unseen instructions. This generality is largely attributed to the incorporation of large language models (LLMs) and vision-language models (VLMs), which provide robust understanding capabilities for interpreting given instructions. For instance, pioneering works introduced the concept of VLM-based robot action generation. Subsequently, studies like OpenVLA \cite{kim2024openvla} and LLARVA \cite{niu2024llarva} have further demonstrated the feasibility and effectiveness of this approach.

Third, data synthesis techniques have also played a significant role. Recent studies have adopted diffusion models for prediction instead of traditional regression or classification methods. Diffusion models are renowned for generating realistic and diverse data, and VLA studies exploit this property to predict plausible and varied robot actions. This approach enhances the model's ability to handle a wide range of scenarios, contributing to more robust and adaptable robotic behaviors.

Despite these advancements, a critical drawback of current VLA methods is the processing time. LLMs demand substantial computational resources, and the cost escalates with the length of the instruction. When these models are applied to practical robots, the resultant motions often appear unnatural and discontinuous due to computational delays. This limitation hampers the real-time applicability of VLA models in dynamic environments where swift and smooth robot actions are essential.

In this paper, we leverage the concepts of modular design inspired from the structure of the human brain to partition the VLA process into multiple distinct modules: (1) a basic sensory module, (2) an intention module, (3) a lightweight module for predicting intermediate actions, and (4) motor module. The sensory module basically process the given input data such as text and image. The intention module focuses on comprehending long-term components such as the task instruction and the initial environmental observations. The third module processes short-term components, including the current motion and visual inputs. The last one practically excutes the predicted action. By strategically scheduling these modules—processing the intention module less frequently and the others more frequently—we reduce redundant computations and enhance the naturalness of the robot's motions. This approach aims to balance the depth of understanding with computational efficiency, thereby improving the real-time performance of VLA models in practical robotic applications.

\section{Problem}
As previously mentioned, prior VLA methods suffer from heavy computational demands, leading to unnatural and discontinuous robot actions. For example, RT-2 \cite{brohan2023rt} reported that their 55B model operates at frequencies between 1 and 3 Hz, while their 5B model runs at approximately 5 Hz under their experimental settings. Similarly, OpenVLA \cite{kim2024openvla} achieves processing speeds of 6 Hz on a single NVIDIA RTX 4090 GPU. To attain optimal performance, robots using these models must pause every 1/6 of a second to predict the next action. Although parallelization can somewhat smooth these discontinuities, it often comes at the expense of reduced task success rates.

Furthermore, it is well-known that diffusion processes involve multi-step sequential denoising procedures, which inherently result in slow generation times. This issue has been extensively discussed in the literature, and several studies have attempted to accelerate the process with minimal loss in the quality of generated data. For instance, DDIM \cite{songdenoising} reformulated the standard diffusion process using the Euler method, while PNDM \cite{liupseudo} and DPM++ \cite{lu2022dpm} applied linear multistep methods to reduce the number of required iterations. As a result, methods like Diffusion Policy \cite{chi2023diffusion} and Octo \cite{team2024octo} inherit these computational challenges and suffer from slow generation times.

As demonstrated, recent approaches require substantial computational resources, leading to slow processing times and discontinuous actions. In practical scenarios, such discontinuous motion can be unsettling for users and detract from the overall user experience. Therefore, there is a pressing need to develop faster VLA methods that can produce smooth and natural robot actions without compromising performance or task success rates.

% As mentioned, prior VLA must suffer from the heavy computation, leading the unnatural and discontinuous robot actions. For example, RT-2 \cite{} stated that their 55B model can run with 1 to 3 Hz and 5B model work with about 5Hz frequency under their setting. Then, OpenVLA \cite{} can be processed with 6Hz on a single NVIDIA 4090. For the best performance, robots must stop for every 1/6 second to predict the next action. By parallelization, it can be more smooth, but sacrifice some task success rate.  

% Further, it is widely known that diffusion process is composed of multi-step sequential denoising process, requiring slow generation. This issue has been widely pointed and there have been several studies to accelerate with small damage in quality of generated data. For instance, DDIM \cite{} reformulated the naive diffusion process to Euler method and PNDM \cite{}, DPM++ \cite{} applied linear multistep method for reducing the number of required iterations. Diffusion policy \cite{} and Octo \cite{} must inherit this issue, so they should suffer from the slow generation. 

% As shown, recent approaches need high computation, leading the slow processing time and discontinuous action. Considering the practical scenario, the discontinuous motion gives uncomfort to users. Therefore, it is required to develop a fast way of VLA. 


==> tex/method_motivation.tex <==
\subsection{Motivation}
\label{sec:motivation}


\begin{figure}[!t]
	\centering
    \begin{minipage}{0.7\linewidth}
	    \centering
	    {\includegraphics[width=1.\textwidth]{./Figures/Decomposition.png}}  
    \end{minipage}%
\caption{\small Schematic of our approach.\textcolor{red}{(This picture is somewhat meaningless.)}}\label{fig:schematic}
\end{figure}

We drew inspiration for our solution from the structure of the human brain. According to the literature \cite{virameteekul2022we}, the human brain is composed of several cortical regions, each with its own functionality. Among these distinct regions, there are the sensory cortex, planning cortex, and motor cortex. Human motions are generated through the harmonization of these separate functions, with the regions operating in parallel.

Leveraging these separate functionalities, we designed our approach to divide the overall function into multiple sub-functions: (1) sensory processing, (2) intention decision, (3) motion planning, and (4) motor control, as illustrated in Figure \ref{fig:schematic}. It is noteworthy that the positioning of each function in Figure \ref{fig:schematic} corresponds to the locations of the functional cortices in the brain. This division allows for parallel processing of modules, similar to how different regions of the brain operate simultaneously, thereby enhancing efficiency and responsiveness. By separating these functions, it becomes unnecessary to run the intention module at every time step. In contrast, the motor control function should be processed at every time step.

Based on this concept, we utilized a LLM as the intention module, which is processed at a low frequency. We then employed an image encoder as the sensory module, which is processed at every time step, and the encoded features are fed into all other modules as input. Finally, the short-term planning and motor modules receive the determined intention and current encoded features, and output the intermediate robot actions. This modular design not only reduces redundant computations but also enables smoother and more natural robot motions, addressing the limitations of previous VLA methods that suffer from slow processing times and discontinuous actions. With this scheduling, it becomes possible to run the intention module less frequently over many time steps, thereby improving computational efficiency without sacrificing performance.


% We found the solution from the structure of human brain. According to some literature \cite{virameteekul2022we}, human brain is composed of several cortex regions, and each region has its own functionality. Among the separated regions, there exist sensory cortex, planning cortex, and motor cortex. Human motions are generated by harmonization of the separated functions, and the regions work in parallel. 
% Leveraging this separate functionalities, we designed our approach to divide the entire function to multiple sub-functions: 1) Sensory, 2) intention decision, 3) motion planning, and 4) motor control as shown in Figure \ref{fig:schematic}. Please note that the positioning of each function in Figure \ref{fig:schematic} is matched the locations of functional cortex. Once separation, it is redundant to run the intention module for every time-step. In contrast, the motor control function should be processed for ever step. 

% Based on this thought, we used LLM as the intention module, which is processed with low frequency. Then, we employed an image encoder as sensory module, which should be processed for every timestep, and the encoded features become fed into all other modules as input. Last, short-term planning and motor modules receive the decided intention and current encoded features, and return the intermediate robot action. By this scheduling, it is possible to run the intention module for many timesteps.

%===============================================================================


==> tex/related_work.tex <==
\subsection{Vision Language Action}

% \textcolor{red}{(OpenVLA's Related Works): A number of works have explored the use of LLM and VLM for robotic policy learning, e.g., for visual state representations [12, 13], object detection [67], high-level planning [16], and for providing a feedback signal [68–71]. Others integrate VLMs directly into end-to-end visuomotor manipulation policies [14, 15], but incorporate significant structure into the policy architecture or require calibrated cameras, which limits their applicability. A number of recent works have explored similar recipes to ours and directly fine-tuned large pretrained VLMs for predicting robot actions [1, 7, 17, 18, 72–74]. Such models are often referred to as vision-language-action models (VLAs), since they fuse robot control actions directly into VLM backbones. This has three key benefits: (1) it performs alignment of pretrained vision and language components on a large, Internetscale vision-language dataset, (2) the use of a generic architecture, not custom-made for robot control, allows us to leverage the scalable infrastructure underlying modern VLM training [75–77] and scale to training billion-parameter policies with minimal code modifications, and (3) it provides a direct pathway for robotics to benefit from the rapid improvements in VLMs. Existing works on VLAs either focus on training and evaluating in single robot or simulated setups [72–74, 78] and thus lack generality, or are closed and do not support efficient fine-tuning to new robot setups [1, 7, 17, 18].} Most closely related, RT-2-X [1] trains a 55B-parameter VLA policy on the Open X-Embodiment dataset and demonstrates state-of-the-art generalist manipulation policy performance. However, our work differs from RT-2-X in multiple important aspects: (1) by combining a strong open VLM backbone with a richer robot pretraining dataset, OpenVLA outperforms RT-2-X in our experiments while being an order of magnitude smaller; (2) we thoroughly investigate fine-tuning of OpenVLA models to new target setups, while RT-2-X does not investigate the fine-tuning setting; (3) we are the first to demonstrate the effectiveness of modern parameter-efficient fine-tuning and quantization approaches for VLAs; and (4) OpenVLA is the first generalist VLA that is open-source and thus supports future research on VLA training, data mixtures, objectives, and inference.


\textcolor{red}{ChatGPT Generated: The development of VLA has significantly advanced the field of robotics by integrating vision, language, and action policies to enable robots to interact with and understand their environments more effectively. Recent studies have focused on LLM and VLM to enhance the ability of robots to interpret visual scenes, comprehend instructions, and execute appropriate actions.
One of the most influential lines of research in VLA-based robot policy learning is the Robot Transformer series. Robot Transformer 1 \cite{brohan2022rt} introduced the concept of multi-modal transformers that can process both visual and linguistic data, providing a unified framework for task understanding. It demonstrated that transformers could capture complex dependencies between sensory inputs and task-specific actions. Robot Transformer 2 \cite{brohan2023rt} expanded this framework by incorporating a self-attention mechanism across visual and linguistic modalities, improving the robot’s ability to parse ambiguous instructions and reason about its surroundings in more dynamic settings. The evolution continued with Robot Transformer X, which introduced a hierarchical architecture that integrates low-level sensory inputs with high-level planning capabilities, further enhancing the precision of robotic actions in real-world environments.
OpenVLA represents another key contribution to the VLA domain, focusing on open-source development. OpenVLA provided an extensible framework that allows researchers to develop and train robots in simulated environments using pre-trained LLMs and VLMs, making it a cornerstone for community-driven research. It emphasizes the interoperability between diverse data sources and models, fostering rapid experimentation with vision-language-action tasks in robotic systems.
In parallel, Octo \cite{team2024octo} offers an alternative approach by focusing on scalability in multi-task learning scenarios. Octo’s architecture is designed to handle a wide range of tasks across different environments, learning from diverse datasets that span various visual and linguistic challenges. This versatility allows it to generalize across tasks that require combining object recognition, language understanding, and action execution, making it one of the most adaptive models in VLA-based robotics.
Another important line of research in this field is Diffusion Policy \cite{chi2023diffusion}, which diverges from transformer-based architectures and introduces diffusion models for action policy learning. By modeling the stochastic nature of real-world environments, Diffusion Policy allows robots to generate more robust and adaptive action sequences in tasks requiring continuous, high-dimensional control. This probabilistic approach enhances the reliability of robots in complex manipulation and navigation tasks where uncertainty and variability are inherent.
Together, these works represent the cutting edge in VLA-based robot action policy. By leveraging the power of LLMs and VLMs, they have demonstrated the potential to revolutionize how robots perceive, understand, and interact with the world, leading to more autonomous and intelligent systems capable of handling a wide variety of real-world tasks.}
